Gaussian Process Regression of Steering Vectors With Physics-Aware Deep Composite Kernels for Augmented Listening

This paper investigates continuous representations of steering vectors over frequency and microphone/source positions for augmented listening (e.g., spatial filtering and binaural rendering), enabling user-parameterized control of the reproduced sound field. Steering vectors have typically been used for representing the spatial response of a microphone array as a function of the look-up direction. The basic algebraic representation of these quantities assuming an idealized environment cannot deal with the scattering effect of the sound field. One may thus collect a discrete set of real steering vectors measured in dedicated facilities and super-resolve (i.e., upsample) them. Recently, physics-aware deep learning methods have been effectively used for this purpose. Such deterministic super-resolution, however, suffers from the overfitting problem due to the non-uniform uncertainty over the measurement space. To solve this problem, we integrate an expressive representation based on the neural field (NF) into the principled probabilistic framework based on the Gaussian process (GP). Specifically, we propose a physics-aware composite kernel that models the directional incoming waves and the subsequent scattering effect. Our comprehensive comparative experiment showed the effectiveness of the proposed method under data insufficiency conditions. In downstream tasks such as speech enhancement and binaural rendering using the simulated data of the SPEAR challenge, the oracle performances were attained with less than ten times fewer measurements.

==> tables/metrics_enhance.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\newcommand{\btt}[1]{#1$^{*}$}
\newcommand{\BST}[1]{\textbf{#1}}
\newcommand{\SEC}[1]{\textbf{#1}}


\begin{tabular}{@{}rccccc|ccccc|ccccc|ccccc|ccccc|ccccc@{}}
% \begin{tabular}{@{}rccccc|cccc|cccc|cccc|cccc|cccc@{}}
\toprule
\multicolumn{1}{c}{}  
 & \multicolumn{5}{c|}{\textbf{SDR impr.} $\uparrow$ [dB]} 
 & \multicolumn{5}{c|}{\textbf{SAR impr.} $\uparrow$ [dB]} 
 & \multicolumn{5}{c|}{\textbf{ISR impr.} $\uparrow$ [dB]}
 & \multicolumn{5}{c|}{\textbf{fwSegSNR impr.} $\uparrow$ [dB]}
 & \multicolumn{5}{c|}{\textbf{PESQ impr.} $\uparrow$}
 & \multicolumn{5}{c}{\textbf{MBSTOI impr.} $\uparrow$} 
 \\ \midrule
\BST{Up. factor }                 
 & 8    & 16   & 32   & 64   & 128 
 & 8    & 16   & 32   & 64   & 128  
 & 8    & 16   & 32   & 64   & 128  
 & 8    & 16   & 32   & 64   & 128  
 & 8    & 16   & 32   & 64   & 128  
 & 8    & 16   & 32   & 64   & 128  
\\ \midrule
\texttt{NN}                    
    & 4.32 & 4.26 & 4.57 & 4.82 & 4.85 
    & 3.33 & 3.51 & 3.51 & 3.75 & 3.88 
    & 2.06 & 1.94 & 2.22 & 2.41 & 2.41 
    & \BST{0.62} & \BST{0.63} & \BST{0.83} & 1.02 & 1.04 
    & \BST{0.03} & 0.03 & 0.03 & 0.03 & 0.03 
    & 0.04 & 0.04 & 0.05 & 0.07 & 0.09 \\
\texttt{SP}
    & 4.47 & 4.69 & 4.89 & 4.97 & 4.98 
    & \BST{3.72} & \BST{3.88} & 4.03 & 4.15 & 4.11 
    & 2.13 & 2.23 & 2.40 & 2.47 & 2.52 
    & 0.61 & 0.59 & 0.79 & \BST{1.04} & \BST{1.11}
    & \BST{0.03} & 0.03 & 0.03 & 0.03 & 0.03 
    & \BST{0.07} & \BST{0.08} & \BST{0.09} & \BST{0.11} & \BST{0.12} \\
\texttt{SH}
    & 4.48 & 4.88 & 4.97 & 5.06 & 5.01
    & 2.57 & 3.78 & 4.00 & 4.02 & 4.08
    & 1.88 & 2.37 & 2.45 & 2.53 & 2.53
    & 0.37 & 0.49 & 0.71 & 0.97 & 1.05
    & 0.02 & 0.03 & 0.03 & 0.03 & 0.03
    & 0.03 & \BST{0.08} & \BST{0.09} & 0.10 & 0.11 \\
\texttt{NF-GW}
    & 5.45 & \btt{5.69} & \btt{6.01} & \btt{6.28} & \btt{7.23}
    & 2.68 & 2.49 & 2.69 & 2.19 & 2.94 
    & 2.64 & 2.83 & 2.98 & \btt{3.11} & \btt{3.90}
    & 0.10 & 0.10 & 0.28 & 0.22 & 0.54 
    & 0.02 & 0.02 & 0.02 & 0.03 & 0.04 
    & 0.05 & 0.05 & 0.04 & 0.02 & 0.05 \\
\texttt{PINN}
    & \btt{5.71} & \btt{5.69} & 6.02 & 5.81 & 5.61 
    & 2.63 & 2.59 & 2.75 & 2.65 & 2.71 
    & 2.77 & 2.79 & 2.93 & 2.87 & 2.76 
    & 0.07 & 0.09 & 0.22 & 0.15 & 0.16 
    & 0.02 & 0.02 & 0.03 & 0.02 & 0.02 
    & 0.05 & 0.05 & 0.04 & 0.04 & 0.05 \\
\texttt{PCNN}
    & \btt{\BST{7.61}} & \btt{\BST{8.64}} & \btt{\BST{8.38}} & \btt{\BST{8.66}} & \btt{\BST{8.57}}
    & 0.50 & 0.28 & 0.92 & 0.82 & 2.16 
    & \btt{\BST{4.32}} & \btt{\BST{4.78}} & \btt{\BST{4.54}} & \btt{\BST{4.92}} & \btt{\BST{4.71}} 
    & 0.04 & 0.19 & 0.26 & 0.30 & 0.57 
    & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 
    & -0.03&-0.04 &-0.02 & -0.01& 0.02 \\
\texttt{GP-Chmat}
    & 5.04 & 5.04 & 5.04 & 5.04 & 5.04 
    & 2.55 & 2.55 & 2.55 & 2.55 & 2.55 
    & 2.48 & 2.48 & 2.48 & 2.48 & 2.48 
    & 0.12 & 0.12 & 0.13 & 0.12 & 0.12 
    & 0.02 & 0.02 & 0.02 & 0.02 & 0.02 
    & 0.06 & 0.06 & 0.06 & 0.06 & 0.06 \\
\BST{\texttt{GP-Steerer}}
    & \btt{7.00} & \btt{6.95} & \btt{6.64} & \btt{6.16} & \btt{6.22}
    & 3.43 & 3.51 & \BST{4.06} & \BST{4.19} & \BST{4.34}
    & \btt{3.64} & \btt{3.59} & \btt{3.62} & \btt{3.37} & \btt{3.35} 
    & 0.61 & 0.47 & 0.71 & 0.93 & 1.10 
    & \BST{0.03} & \btt{\BST{0.05}} & \btt{\BST{0.05}} & \btt{\BST{0.05}} &\btt{\BST{0.05}}
    & 0.05 & 0.06 & 0.07 & 0.09 & 0.09 \\
\midrule
\texttt{NN-Oracle}
    & \multicolumn{5}{c|}{5.61}         
    & \multicolumn{5}{c|}{4.64}         
    & \multicolumn{5}{c|}{3.00}         
    & \multicolumn{5}{c|}{1.20}         
    & \multicolumn{5}{c|}{0.04}         
    & \multicolumn{5}{c}{0.13}             
\\ \bottomrule
\end{tabular}


==> tables/sota_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{lll|llllll}
\toprule
    &                                &                     & \multicolumn{6}{c}{Problems related to steering vector interpolation}                                                                                                                              \\
\multicolumn{3}{c|}{Approaches}                    & \multicolumn{2}{c|}{User-centred sound field}                                  & \multicolumn{4}{c}{Generic sound field}                                                                           \\

& & & \multicolumn{1}{l|}{HRTF upsampling} & \multicolumn{1}{l|}{Source directivity} & \multicolumn{1}{l|}{SFR} & \multicolumn{1}{l|}{HOA mic} & \multicolumn{1}{l|}{RIR interpolation} & Array manifold \\
\midrule

& &  \multicolumn{1}{r|}{\textit{Review papers}}
& \multicolumn{1}{l|}{\cite{porschmann2020comparison,bruschi2024review}} 
& \multicolumn{1}{l|}{} 
& \multicolumn{1}{l|}{\cite{pezzoli2022deep,koyama2024physics}} 
& \multicolumn{1}{l|}{} 
& \multicolumn{1}{l|}{} 
&  \\
\hline

\multirow{5}{*}{\rotatebox[origin=c]{90}{Data-driven}}      
        & \multicolumn{2}{l|}{Weighted interpolation}          
        & \multicolumn{1}{l|}{\cite{hartung1999comparison,begault20003D,gamper2013head,cuevas20193D,ben2020localization,srivastava2020spatial,acosta2020bilinear}} % HRTF
        & \multicolumn{1}{l|}{} % Source directivity
        & \multicolumn{1}{l|}{} % SFR
        & \multicolumn{1}{l|}{} % HOA  
        & \multicolumn{1}{l|}{} % RIR interp            
        &                       % Array
        \\
        
        & \multicolumn{2}{l|}{Subspace methods}
        & \multicolumn{1}{l|}{\cite{kistler1992model,chen1995spatial,larcher2000study,freeland2002efficient,wang2009head,xie2012recovery,zhang2020modeling,torres2009hrtf}}                
        & \multicolumn{1}{l|}{}                   
        & \multicolumn{1}{l|}{}    
        & \multicolumn{1}{l|}{}        
        & \multicolumn{1}{l|}{}                  
        &                
        \\
                                                            
        & \multicolumn{2}{l|}{Deep learning}                   
        & \multicolumn{1}{l|}{\cite{jiang2023modeling,gebru2021implicit,chen2019autoencoding,lee2023global,miccini2020hrtf,zhi2022towards,siripornpitak2022spatial,hogg2023exploring,hogg2023hrtf}}         
        & \multicolumn{1}{l|}{}                   
        & \multicolumn{1}{l|}{\cite{lluis2020sound,kristoffersen2021deep,fernandez2023generative,pezzoli2022deep,miotello2024reconstruction}}    
        & \multicolumn{1}{l|}{}        
        & \multicolumn{1}{l|}{}                  
        &                
        \\

        & \multicolumn{2}{r|}{$\ldots$ with Neural Fields}                   
        & \multicolumn{1}{l|}{\cite{gebru2021implicit,zhang2023hrtf,lee2023neural}}         
        & \multicolumn{1}{l|}{}                   
        & \multicolumn{1}{l|}{}    
        & \multicolumn{1}{l|}{}        
        & \multicolumn{1}{l|}{}                  
        &   
        \\             
        
        & \multicolumn{2}{l|}{Manifold Learning}                   
        & \multicolumn{1}{l|}{\cite{duraiswami2005manifolds,deleforge2015acoustic,grijalva2017interpolation}}
        & \multicolumn{1}{l|}{}                   
        & \multicolumn{1}{l|}{}    
        & \multicolumn{1}{l|}{}        
        & \multicolumn{1}{l|}{}                  
        &                
        \\ \hline


\multirow{7}{*}{\rotatebox[origin=c]{90}{Knowledge-driven}} 
    & \multicolumn{2}{l|}{Geometric-based}                 
        & \multicolumn{1}{l|}{\cite{pulkki1997virtual,franck2017sparse,chen1993synthesis,nishino1999interpolating,carlile2002performance,jenison1996spherical,luo2013kernel,chen2023headrelated,thuillier2024hrtf}}
        & \multicolumn{1}{l|}{}                   
        & \multicolumn{1}{l|}{\cite{lubeck2023spatial,del2011generating,pezzoli2018reconstruction,haneda1994arma}}
        & \multicolumn{1}{l|}{}       
        & \multicolumn{1}{l|}{}                  
        &                
        \\
                                  
        & \multicolumn{2}{l|}{Parametric (DSP)-based}          
        & \multicolumn{1}{l|}{\cite{runkle1995comparison,watanabe2003interpolation,ramos2013parametric,al2019head,queiroz2010structured,nowak2022spatial,lee2022neural,masuyama2024niirf}}                
        & \multicolumn{1}{l|}{\cite{pezzoli2018reconstruction}}
        & \multicolumn{1}{l|}{\cite{murata2016sparse,zea2019compressed}}   
        & \multicolumn{1}{l|}{}        
        & \multicolumn{1}{l|}{}                  
        &                
        \\

        & \multirow{4}{*}{\rotatebox[origin=c]{90}{Physics-based}} 
        & Physics-constrained 
        & \multicolumn{1}{l|}{\cite{ajdler2008sound,evans1998analyzing,duraiswami2004interpolation,zotkin2009regularized,ahrens2012hrtf,porschmann2019directional,zaunschirm2018binaural,ben2019efficient,arend2021assessing}}                
        & \multicolumn{1}{l|}{}
        & \multicolumn{1}{l|}{\cite{samarasinghe2015efficient,pezzoli2022sparsity,koyama2019sparse,damiano2021soundfield,ueno2018kernel,ribeiro2024sound,mignot2013low,bertin2015compressive,antonello2017room,antonello2018room,das2021room}}
        & \multicolumn{1}{l|}{}
        & \multicolumn{1}{l|}{}                  
        &                
        \\

        & 
        & \multicolumn{1}{r|}{$\ldots$ with DNN}
        & \multicolumn{1}{l|}{\cite{ito2022head}}                
        & \multicolumn{1}{l|}{}
        & \multicolumn{1}{l|}{\cite{bi2024point,karakonstantis2023generative,ribeiro2024sound}}
        & \multicolumn{1}{l|}{}
        & \multicolumn{1}{l|}{}
        &                
        \\

        & 
        & \multicolumn{1}{r|}{$\ldots$ with GP}
        & \multicolumn{1}{l|}{\cite{romigh2015bayesian}}                
        & \multicolumn{1}{l|}{}
        & \multicolumn{1}{l|}{\cite{caviedes2021gaussian,caviedes2023spatio,feng2024room}}
        & \multicolumn{1}{l|}{}
        & \multicolumn{1}{l|}{}                  
        &                
        \\
        
        &                                
        & Physics-informed    
        & \multicolumn{1}{l|}{\cite{ma2023physics,ma2024sound}}            
        & \multicolumn{1}{l|}{}         
        & \multicolumn{1}{l|}{\cite{pezzoli2022implicit,shigemi2022physics,chen2023sound,ma2024sound,olivieri2024physics,karakonstantis2024room,middleton2023application,borrel2024sound}}  
        & \multicolumn{1}{l|}{\cite{miotello2024physics}}   
        & \multicolumn{1}{l|}{}       
        &           
        \\
        
        & & 
        & \multicolumn{1}{l|}{}               
        & \multicolumn{1}{l|}{}         
        & \multicolumn{1}{l|}{}  
        & \multicolumn{1}{l|}{}  
        & \multicolumn{1}{l|}{}    
        &              
        \\
    
        \bottomrule
\end{tabular}


==> tables/sota_table_extended.tex <==
\begin{tabular}{
    p{0.03\linewidth}%
    p{0.05\linewidth}%
    p{0.3\linewidth}%
    p{0.22\linewidth}%
    p{0.25\linewidth}}%
\toprule
\multicolumn{3}{c}{}
    & \multicolumn{1}{l}{HRTF upsampling} 
    & \multicolumn{1}{l}{Sound Field Reconstr.} 
    \\
\midrule

\multicolumn{3}{c}{Recent reviews}
    & \multicolumn{1}{l}{\cite{porschmann2020comparison,bruschi2024review,cobos2022overview}}
    & \multicolumn{1}{l}{\cite{koyama2024physics,cobos2022overview}} 
    \\[0.5ex]
\hline\\

\multirow{5}{*}{\rotatebox[origin=c]{90}{Data-driven}}      
        & \multicolumn{2}{l}{Local interpolation}          
        & \multicolumn{1}{l}{\cite{freeland2002efficient,begault20003D,gamper2013head,cuevas20193D,porschmann2020comparison}} % HRTF
        & \multicolumn{1}{l}{$\sim$} % SFR
        \\
        
        & \multicolumn{2}{l}{(Global) Subspace  methods}
        & \multicolumn{1}{l}{\cite{kistler1992model,torres2009hrtf,xie2012recovery}}                % HRTF
        & \multicolumn{1}{l}{$\sim$}   % SFR 
        \\
                                                     
        & \multicolumn{2}{l}{Deep learning}           
        & \multicolumn{1}{l}{\cite{jiang2023modeling,gebru2021implicit,hogg2023exploring,hogg2024hrtf}} % HRTF
        & \multicolumn{1}{l}{\cite{lluis2020sound,kristoffersen2021deep,
        % fernandez2023generative,
        pezzoli2022deep,miotello2024reconstruction}}     % SFR
        \\             

        & \multicolumn{2}{r}{$\ldots$ with multimodalies}    
        & \multicolumn{1}{l}{\cite{chen2019autoencoding,lee2023global,miccini2020hrtf,zhi2022towards}}                     % HRTF
        & $\sim$
        \\
        & \multicolumn{2}{r}{$\ldots$ with Neural Fields}
        & \multicolumn{1}{l}{\cite{gebru2021implicit,zhang2023hrtf,lee2023neural}} % HRTF
        & \multicolumn{1}{l}{$\sim$}     % SFR
        \\[3pt]
        
        & \multicolumn{2}{l}{Manifold Learning}
        & \multicolumn{1}{l}{\cite{duraiswami2005manifolds,deleforge2015acoustic,grijalva2017interpolation}} % HRTF
        & \multicolumn{1}{l}{}    % SFR
        \\[2pt] \hline

\multirow{7}{*}{\rotatebox[origin=c]{90}{Knowledge-driven}} 
    & \multicolumn{2}{l}{Geometric-based}                 
        & \multicolumn{1}{l}{\cite{pulkki1997virtual,franck2017sparse,chen1993synthesis,nishino1999interpolating,jenison1996spherical,luo2013kernel,chen2023head,thuillier2024hrtf,zotkin2009regularized,wang2009head}} % HRTF
        & $\sim$
        \\
                                  
        & \multicolumn{2}{l}{Parametric (DSP)-based}          
        & \multicolumn{1}{l}{\cite{runkle1995comparison,watanabe2003interpolation,al2019head,nowak2022spatial,lee2023neural,masuyama2024niirf}}
        & $\sim$
        \\[3pt]

        & \multirow{4}{*}{\rotatebox[origin=c]{90}{Physics-{\scriptsize based}}} 
        & Physics-constrained 
        & \multicolumn{1}{l}{\cite{ajdler2008sound,evans1998analyzing,duraiswami2004interpolation,zotkin2009regularized,ahrens2012hrtf,porschmann2019directional,zaunschirm2018binaural,ben2019efficient,arend2021assessing}}
        & \multicolumn{1}{l}{\cite{mignot2013low,bertin2015compressive,ueno2018kernel,koyama2019sparse,damiano2021soundfield,caviedes2021gaussian,ribeiro2024sound,samarasinghe2015efficient,pezzoli2022sparsity,grande2019sound,das2021room,antonello2017room}}%
        \\

        & 
        & \multicolumn{1}{r}{$\ldots$ with DNN}
        & \multicolumn{1}{l}{\cite{ito2022head}}      
        & \multicolumn{1}{l}{\cite{karakonstantis2023generative,ribeiro2024sound,feng2024room,bi2024point}}
        \\

        & 
        & \multicolumn{1}{r}{$\ldots$ with GP}
        & \multicolumn{1}{l}{\cite{luo2013kernel,romigh2015bayesian}}
        & \multicolumn{1}{l}{\cite{caviedes2021gaussian,caviedes2023spatio,feng2024room}}
        \\
        
        &                                
        & Physics-informed    
        & \multicolumn{1}{l}{\cite{ma2023physics}}
        & \multicolumn{1}{l}{\cite{pezzoli2023implicit,shigemi2022physics,chen2023sound,ma2024sound,miotello2024physics,olivieri2024physics,karakonstantis2024room,middleton2023application,veerababu2024neural,borrel2024sound}}  
        \\
        
        & & 
        & \multicolumn{1}{l}{}               
        & \multicolumn{1}{l}{}  
        \\
    
        \bottomrule
\end{tabular}


==> tikz_figures/biblio_scheme.tex <==
% % I am using only the basic, xnode, and tnode styles
% \tikzset{
%     basic/.style  = {draw, text width=3cm, align=center, font=\sffamily, rectangle},
%     root/.style   = {basic, rounded corners=2pt, thin, align=center, fill=green!30},
%     onode/.style = {basic, thin, rounded corners=2pt, align=center, fill=green!60,text width=3cm,},
%     tnode/.style = {basic, thin, align=left, fill=pink!60, text width=15em, align=center},
%     xnode/.style = {basic, thin, rounded corners=2pt, align=center, fill=blue!20,text width=5cm,},
%     wnode/.style = {basic, thin, align=left, fill=pink!10!blue!80!red!10, text width=6.5em},
%     edge from parent/.style={draw=black, edge from parent fork right}

% }
% %

% \begin{forest} for tree={
%     grow=east,
%     growth parent anchor=west,
%     parent anchor=east,
%     child anchor=west,
%     edge path={\noexpand\path[\forestoption{edge},->, >={latex}] 
%          (!u.parent anchor) -- +(10pt,0pt) |-  (.child anchor) 
%          \forestoption{edge label};}
% }
% % l sep is used for arrow distance
% [Reconnaissance Survey, basic,  l sep=10mm,
%     [Network Scanning, xnode,  l sep=10mm,
%         [Shaikh et al.\, 2008, tnode]
%         [Bhuyan et al.\, 2011, tnode]
%         [Bou et al.\, 2013, tnode] ]
%     [Social Engineering, xnode,  l sep=10mm,
%         [Chiew et al.\, 2018, tnode]
%         [Heartfield \& Loukas\, 2015, tnode]
%         [Salahdine et al.\, 2019, tnode] 
%         [Alharthi et al.\, 2020, tnode] ]
%     [Open-Source Footprinting, xnode,  l sep=10mm,
%         [Rai et al.\, 2021, tnode]
%         [Kanta et al.\, 2020, tnode]
%         [Glassman et al.\, 2012, tnode] 
%          ] ]
% \end{forest}


\tikzset{
  basic/.style  = {draw, text width=2cm, drop shadow, font=\sffamily, rectangle},
  root/.style   = {basic, rounded corners=2pt, thin, align=center, fill=white},
  level-2/.style = {basic, rounded corners=6pt, thin,align=center, fill=white, text width=3cm},
  level-3/.style = {basic, thin, align=center, fill=white, text width=1.8cm}
}

\begin{tikzpicture}[
  level 1/.style={sibling distance=12em, level distance=5em},
  % {edge from parent fork down},
  edge from parent/.style={->,solid,black,thick,sloped,draw}, 
  edge from parent path={(\tikzparentnode.south) -- (\tikzchildnode.north)},
  >=latex, node distance=1.2cm, edge from parent fork down]

% root of the the initial tree, level 1
\node[root] {\textbf{Spatial sound upsampling}}
% The first level, as children of the initial tree
  child {node[level-2] (c1) {\textbf{HRTF upsampling}}}
  child {node[level-2] (c2) {\textbf{Sound Field Reconstitution}}}
  child {node[level-2] (c3) {\textbf{RIR estimation}}}
  child {node[level-2] (c4) {\textbf{Category 4}}};

% The second level, relatively positioned nodes
\begin{scope}[every node/.style={level-3}]
\node [below of = c1, xshift=10pt] (c11) {item 1-1};
\node [below of = c11] (c12) {Weighted interpolation};
\node [below of = c12] (c13) {Subspace methods};
\node [below of = c13] (c14) {Deep neural networks};

\node [below of = c2, xshift=10pt] (c21) {item 2-1};
\node [below of = c21] (c22) {item 2-2};
\node [below of = c22] (c23) {item 2-3};
\node [below of = c23] (c24) {item 2-4};

\node [below of = c3, xshift=10pt] (c31) {item 3-1};
\node [below of = c31] (c32) {item 3-2};
\node [below of = c32] (c33) {item 3-3};
\node [below of = c33] (c34) {item 3-4};
\node [below of = c34] (c35) {item 3-5};

\node [below of = c4, xshift=10pt] (c41) {item 4-1};
\node [below of = c41] (c42) {item 4-2};
\end{scope}

% lines from each level 1 node to every one of its "children"
\foreach \value in {1,2,3}
  \draw[->] (c1.195) |- (c1\value.west);

\foreach \value in {1,...,4}
  \draw[->] (c2.195) |- (c2\value.west);

\foreach \value in {1,...,5}
  \draw[->] (c3.195) |- (c3\value.west);
  
\foreach \value in {1,2}
  \draw[->] (c4.195) |- (c4\value.west);
\end{tikzpicture}
